Interactions par franchissement gr\^ace a un syst\`eme de suivi du regard

Human-computer interactions based on gaze-tracking have spread during the last few years. Video games, applications in health, trading, market research, and many other fields have started to use this new technology that seems invisible to the user. However, the dominant form of interaction using gaze tracking uses dwell-time for command activation, which introduces strong constraints in the interaction: dwell-time activation requires users to look steadily at an element for a predefined amount of time in to select it. While dwell-time alleviates a part of the Midas touch problem (referring to the fact that an element fixed by the user will be activated even if it was not intended to do so), it doesn't completely remove it: users should not gaze too long on an item, or they may trigger an unintended activation. In addition, dwell-time slows down users' interaction by requiring a pause each time an activation is needed. In this project, we study an alternative selection method based on crossing interactions, a well-studied method used in conventional HCI. This interaction allows users' gaze to rest in areas that don't have crossing triggers, and it removes the need to pause in the interaction. We found that crossing interaction had similar performances than dwell-time interaction with novice users. The performance was even better for users having previous experience with gaze interaction.

==> Master2Repport/chapters/1_Introduction.tex <==
\chapter{Introduction}

The first studies concerning accurate measures of eye movement appeared around the end of the 19th century with the fruitless attempts in measuring of nystagmus, the involuntary oscillation and saccade movements of the eye, tried by Rählmann   \cite{Raehlmann1878} and Ahrens  \cite{Ahrens1891}. First methods were really invasive and not reliable, they started with an ivory cup on the cornea attached to a bristle connected to a kymograph, improved by Delabarre   \cite{Delabarre1898} or Huey   \cite{Huey1898, Huey1900} from Ahrens method, and then with a plaster-of-Paris eye-cups, which required the eye to be anesthetized with cocaine. Fortunately, huge improvement appeared quickly proposing more and more comfortable and accurate techniques. The currently used techniques are the video-oculography (VOG), video-based tracking using infrared light (IR), pupil-corneal reflection (PCR), and Electrooculography (EOG) methods   \cite{fairclough2014}. From years, eye tracking interactions have been designed by using the dwell-time technique, a technique consisting in activating an item when the user looks at it during a certain amount of time. Unfortunately, there are still some problems with the use of this method. The most famous one being probably the {\em Midas Touch} problem related to the legend of the Greek King Midas, turning everything he touched into gold:
\newline

{\em "And, while he (Midas)[...] tried to bite with hungry teeth a tender bit of meat, the dainty, as his teeth but touched it, shone at once with yellow shreds and flakes of gold. And wine, another gift of Bacchus, when he mixed it in pure water, can be seen in his astonished mouth as liquid gold."} - OVID, METAMORPHOSES 11.
\newline

Hence, the Midas Touch problem, or as Majaranta  \cite{majaranta36} says, the Midas Gaze problem here, refers to the fact that every look at an object is considered as an interaction request, even if the eye movement was not intended to trigger an action. New methods tend to reduce the impact of this problem, for example by adapting the dwell-time automatically, but it is still hard to determine precisely if a look at an object is just an observation from the user or if it has to be considered as a dwell-interaction. The dwell-time is also usually too long to make the user able to use the software in a "comfortable" and "human-like" rhythm. He/She can therefore be disturbed by the fact that his eyes can not rest due to these unwanted actions.

We identify two categories of people using gaze tracking; The people who are usually using eyes as one modality of a multimodality system and in this case, the gaze is just a way of pointing and not a direct way to interact. And, the people using eye-only interaction system, like people with strong motor impairments, for those the gaze is the only available modality and the need of having fast and comfortable interaction with eyes become obviously essential.
\newline \newline
In Human history, people with disabilities have, more or less, always been set aside by their society, structures being unadapted, means of transport, ways of communication, being very precarious or even nonexistent.

After that world wars pointed out at the unsolved situation of handicapped people, at the end of the XXth century mentalities finally started to change and several laws have been created for the rights of disabled people in 1975  \cite{loi75}, 1987   \cite{loi87} and 1990   \cite{loi90}. More precisely, it's only in 2005, the 11th of February, that "the Law on Equal Rights and Opportunities, Participation and Citizenship of Persons with Disabilities"  \cite{loi2005} have been established in France. Still, the laws can be hard to handle for some structures and for the government as the law modification of an important article of this last law showed in 2017   \cite{article11171}, reducing the quota of new accommodation livable by people with disabilities, rising a huge polemic in France. The creation of new systems, allowing more autonomy and more way of interaction with new technologies seems to be something important to work on.
\newline\newline
The idea behind our project is to focus on these people, having strong disabilities, more precisely on people having multiple disabilities, who need to have daily use of these eye-only interaction systems. The definition of "multiple disabilities" is quite recent actually, we can find a good description and history of it in a study from Inserm, for the CNSA, about rare disabilities       {inserm2013}. Elisabeth Zucman, Physician in functional rehabilitation and Honorary President of the \textit{ PolyHANDICAP Group France (GPF)}, used these terms for the first time officially in 1969. In 1979, Salbreux and coll. \cite{salbreux} distinguished three different french terms that still don't really have an English translation: 
\begin{itemize}
\item {\em plurihandicap}: Association of several disabilities that don't have any link together. For the people with this kind of disabilities, mental and cognitive deficiency is never high. (Can be sometimes wrongly translated by "multiple disabilities").
\item {\em surhandicap}: Association of behavioral disorders with other pre-existing severe disabilities or deficiencies.
\item {\em polyhandicap}: Most of the time, it's an association of severe physical and mental disabilities resulting in an extreme autonomy restriction. We will speak about this kind of disabilities in our report, using the term "multiple disabilities".
\end{itemize}

In the same study, the prevalence \footnote{{\em Prevalence} in epidemiology is the proportion of a particular population found to be affected by a medical condition.} rate for the multiple disabilities is denoted as clearly up to 0.2 \%. A more recent study by Arvio and Sillapää \cite{arvio2003} in 2003 in a region of Finland denoted a rate of 0.13 \%. By taking a lower rate, about 0.1\%, and knowing that the European population in 2019 is over 740 million of people, this could lead to 740 000 people possibly having these kinds of disabilities.

Let's imagine that from now you can only speak at the same speed than you're typing on a keyboard. Between each key entry, add half a second more, it seems slow and frustrating, isn't it? Unfortunately, it's almost what some people with strong motor impairments are facing every day. Despite the creation of all the new techniques and technologies, people having strong physical disabilities can express themselves with a word rate going from only 1 to 20 words per minute using gaze, against the usual flow of some 100 words per minutes that valid people can easily handle with voice. Moreover, this "slow-down" problem doesn't occur only in the communication field but also in all the everyday life situations for them who are not able to use their body correctly, for them who need to be daily equipped with eye-tracker and who have to use it with not efficient and not suitable software. Each action, as simpler as it is, each interaction, with objects, with people, can quickly become frustrating and hard to achieve. It can become even harder to propose some suitable software when these people are children with multiple disabilities, who are usually not able to read a text and who have to use picture or pictogram to communicate with others.
\newline

The goal of this study is thus to propose and test an alternative dwell-free interaction method solving the Midas Touch problem and being faster than the usually used Dwell-time method, for people having to use these eye-only systems. We investigate {\em crossing interaction}. Crossing interaction was introduced by Accot in 2002 \cite{accot2002}, its main principle consist in activating an item by crossing a boundary. In particular, it does not require the use of another modality (such as pressing a button) for validation. As crossing a boundary with gaze can be faster than the typical dwell time used for validation, we anticipate faster interaction.
\newline

Our ultimate goal was the evaluation of the benefits of crossing interaction with people having disabilities. However, finding and inviting a sizable number of people with disabilities to participate in a number of experimental sessions did not seem to be tractable in the timeframe of this Master project. In addition, it is common to consider people with no disability as one homogeneous population and to sample randomly in this population. The situation is quite different with disabilities which can vary a lot across individuals, even in the realm of what is categorized as the "same" disability. It exists a lot of different multiple disabilities, for example, having different characteristics (the most frequent ones are presented in Morel's et al.~\cite{morel2017}), so it is important to think about each of them. Angelman and Rett Syndrome are for example two kinds of multiple disabilities, but they have strong differences, and these difference can also vary with the people having the "same" Syndrome, some can have learned how to say a few words when some others can't, some can have a partial use of their legs, some others don't, etc. Because of these difficulties we decided that focusing our study on people without disabilities was a reasonable first step that would still inform on the potential benefits of crossing interactions. Gaze interaction is less common with people without disabilities, but it has its use in various domains, such as surgery where the hands are occupied and cannot be used for human-computer interaction (HCI), or during temporary incapacity following an accident or illness. We anticipate that our study involving people with no disability will inform how crossing interaction could improve HCI for people with disabilities. We keep in mind, however, that these two population may have quite different behaviors and that what we observe will not transfer directly.

The larger objective is to test our design implementation after this Master's project with people with multiple disabilities and on the next step, if the results are conclusive, to use this new way of interaction in the design of a fast pictogram-based augmentative and alternative communication (AAC) system (it's to say a system based on communication methods created to complete or replace speech or writing for people with difficulties in the production or comprehension of spoken or written language) that could be used daily by the children with strong multiple disabilities.
\newline\newline\newline

\textbf{Contributions.} The main contributions of this paper are the following:
\begin{itemize}
\item we designed a state-of-the art of the different studies about crossing method that could be interesting in the adaptation for eye-tracking systems with a background for alternative and augmentative communication with children with multiple disabilities.
\item we proposed a formula to compute the maximal number of slices that can be placed into a circular pie menu usable for eye-trackers.
\item we adapted the crossing interaction method to the eye-tracking technology by creating a design that could be tested easily with children having multiple disabilities.
\item we tested the efficiency of crossing interaction for the Tobii 4C eye-tracker for people with no disabilities having and having not use an eye-tracking device before.
\end{itemize}



==> Master2Repport/chapters/2_Chapter2.tex <==
\chapter{Related Works}

\section{Limitations of dwell-time}

After its entry on the research field, eye tracking technology seems to finally reach the general public. Video games\footnote{Tobii Gaming Website: https://gaming.tobii.com/}, business market\footnote{Tobii Pro in Marketing: https://www.tobiipro.com/fields-of-use/marketing-consumer-research/}  \cite{market2,market3,market1},  surgery\footnote{Tobii Pro in Surgery: https://www.tobiipro.com/fields-of-use/professional-performance/customer-cases/eye-tracking-as-a-way-to-illustrate-surgical-methods-and-assess-students-learning/}, and other working area now have their own eye-tracking devices like Tobii{\copyright}  eye trackers \footnote{Tobii and Tobii Pro Websites: https://www.tobii.com/ ; https://www.tobiipro.com/} for example, with adapted software and well-suitable algorithms like the ones evaluated by Kar \cite{kar2017} in consumer platforms.

Usually mixed with other modalities for people without disabilities, eye-tracking principle allows the user to use his/her gaze as main input entry for pointing, by mapping the eye input directly to a position on the screen, while the other modality such as voice, pedals, etc ... are used for actions like selection.
Some applications are using gaze tracking as the only modality. For some people, being unable to use some hand devices, for example, several fully eye-based software has been designed.

The human gaze is never fixed, it keeps achieving saccade movements, therefore, an extended fixation time can be associated to an explicit request for interaction from the user, it's the idea used by dwell-time principle. Other systems, like the use of anti-saccade studied by Huckauf \cite{huckauf2011} or gaze path by Kurauchi \cite{kurauchi2018} also have been studied but they tend to be less intuitive and slower than dwell-time or can be applied only in a given context (e.g. text-entry with the prediction for gaze path).
The use of blinking or winking is also quite frequently used, but some huge problems are still present with these interactions. Firstly, everybody is not able to blink or wink voluntarily, so this method can't apply to all the people, especially for some people with disabilities who are not in control of their eyes blinking. Secondly, human people usually blink around 10 times per minutes, what makes the explicit of the action less obvious and can lead to unexpected activations. Several methods by forced blink have been tested as Majaranta \cite{majaranta2002} explains, but they lead to an inaccurate action due to the fact that the eyes are "lost" by the eye tracker and they are also leading to a big waste of time.

We will focus our study on people having strong impairments making them capable to only use his/her eyes as input entry. Some of them are unable to control blinking, to use speech or to control their hands and feet. The eyes are hence one of the remaining ways of interaction with these people and the dwell-time is generally considered as the most efficient way to do so.

Several AAC systems and text entry systems usable by eye tracker have been designed these last tenth of years. Majaranta provides a list of some currently available commercial eye control systems targeted at people with disabilities \cite{majaranta36}.

Still, with all these different studies the dwell-time seems to remain the only valuable solution in order to try to compensate the Midas Touch problem by keeping an "acceptable" action speed in a comfortable way for "general" actions (it's to say non-text-entry actions). The biggest problem that occurs when using a dwell-time solution is that each dwell can be considered as wasted time and is breaking the flow of action. Overall, interaction performance is reduced. Moreover, even if dwell action tries to compensate the Midas Touch problem, it is still not perfect at all and needs to be adapted to the user, context, etc... avoiding the user to observe the screen as he/she would like to not unexpectedly activate elements on the screen.

This rise in the use of eye tracking systems, particularly in the field of communication, shows a real and important need for researchers to improve the possible eye-based interactions, the currently proposed interactions remain quite limited: either they are not allowing a total control of the environment by the eye, either they are facing the well-known Midas Touch problem. 



\section{When dwell-free is faster than dwell-based}


In order to stay in an ecological mind, our idea should hence be designed in order to avoid this dwell period, to gain some time on each small interaction that could be implied by the use of an AAC system.
An example of an interaction that is really impacted by this dwell-time period is, for example, the text entry software. For now, using dwell-time on a basic {\em AZERTY} or {\em QWERTY} keyboard is adding a dwell period on each key pressed, what turns the action into a long and boring process. On one side, valid people can easily have a speech conversation of over 100 wpm (words per minutes)as Majaranta explained \cite{majaranta2002}, but on the other side, people using eye tracking system are limited in their word-flow by this problem. A theoretical study from Kistensson \cite{kristensson2012} showed that using an azerty keyboard with a dwell-free interaction and no prediction would lead to a maximum flow of 46 wpm what is more than two times lower than the valid people speech rate.

Fortunately, some dwell-free interactions, using word prediction and uncommon designs, tend to considerably reduce "typing" time. Dasher \cite{dasher2000} is one of the most famous and efficient ones, and even if it can be improved, as noticed by the writers, it can already reach 34 wpm with good training. Eye swipe \cite{kurauchi2016,kurauchi2018} is also an interesting and efficient double crossing method, but it is mainly based on prediction, it is hence hardly applicable for our study that should be usable for a bunch of non-predictable actions.
Some other techniques, while less efficiency than Dasher and Eye Swipe, are actually more interesting for our research. The off-screen version of Isokoski \cite{isokoski2000} was one of the first ideas, but require to subdivide the task into several small action, in this case the time gained by removing the dwell-time is lost by the division of the tasks.

The Quikwriting adaptation of Andr\'e and Bee \cite{andre2008} seems to be really promising with its idea of "hierarchical" selection by crossing, allowing the user to select an element of a section really easily as shown bellow on the fig \ref{quikwriting}. They demonstrated that this method {\em "can easily compete with gaze-controlled keyboard-based systems"}. They explained that {\em "Quikwriting was originally designed for the usage with stylus-based input devices"}. They used the principles of always moving and never lifting the stylus, to match human’s gaze nature and thought that these kind of principle should be considered in others eye based interaction, as we will try to do here.

\begin{figure}[!h]
    \center
    \includegraphics[width=7.5cm]{pics/quikwriting.png}
    \caption{ {\em Adapted interface of Quikwriting for use with eye gaze. The dotted line indicates the gaze path to write the letter ’g’. The user currently looks at ’g’. The light shaded background follows the gaze and indicates which section the user is looking at.} by Andr\'e \cite{andre2008}}
    \label{quikwriting}
\end{figure}

Finally, the nearest idea to our project is probably the pEye implementation by Huckauf \cite{huckauf2007,huckauf20082}, whose basically designed for a text entry application as you can see on the fig \ref{pEyeA} but that has been refined to be used as a more universal input for example for desktop navigation with the pEYEtop \cite{huckauf20081} implementation fig \ref{pEyeTop}. Huckauf proved that pEYEs can be "effectively and efficiently used in tasks requiring lots of selections", as expected in our study, even if the optimal number of slices for a menu of a given size still has to be determined as concluded in the Huckauf and Urbina's paper about pEYE limitations\cite{urbina2010}.

\begin{figure}[h!]
\begin{minipage}{.5\textwidth}
  \centering
  \includegraphics[width=8.5cm]{pics/pEyeA.png}
  \captionof{figure}{Selection of the letter "a" with pEYE. {\em The central pEYE serves
for typing, and on-screen buttons provide other functionalities. The
text is displayed in the the lower part of the screen.} by Huckauf \cite{huckauf2007,huckauf20082}}
  \label{pEyeA}
\end{minipage}%
\hspace{0.1\textwidth}\begin{minipage}{.4\textwidth}
  \centering
  \includegraphics[width=6.5cm]{pics/pEyeTop.png}
  \captionof{figure}{pEYEtop, the desktop file navigator adaptation using pEYE original design\cite{huckauf20081}}
  \label{pEyeTop}
\end{minipage}
\end{figure}


Most of the quoted interactions have been presented in the Huckauf Study \cite{huckauf20082} about computer-gaze interaction, but they are compared regarding text-entry editor idea, what is not exactly the point of our study. 


\section{Crossing Interaction}

We're mainly using mouse device on computer, allowing a selection by left click, or simply our finger on smartphones where touch is the main interaction, but other kinds of selection also exist that only require a single modality for both pointing and activating, our main requirement.
The crossing interaction seems to be one of the most reliable of them, as explained before, the crossing principle is to cross an element in order to trigger an action, for example, crossing an area could activate the corresponding button. 

\begin{figure}[!h]
    \center
    \includegraphics[width=8cm]{pics/crossY.PNG}
    \caption{{\em The correspondence table showing elements of traditional, point-and-click GUIs and their CrossY counterparts.} by Apitz \cite{apitz} }
    \label{crossY}
\end{figure}

Accot's study \cite{accot2002} compared the traditional point-and-click interaction with the crossing interaction by showing that each of them was following a Fitts’s law (cf fig \ref{FittLaw}). This study showed that crossing and point-and-click had Fitts's parameters of similar value for the same kind of task. Crossing was eventually considered as efficient as point-and-click on basic WIMP interface. It can even be interesting with direct touch, as shown by Luo et al. \cite{luo2014}. The direct interactions are usually feeling natural to the user and can be useful to reduce the time needed to activate an object, because there is no intermediate device. Cao et al. \cite{cao2006} also explain in their study that crossing selection techniques can provide quick and fluid interaction with a hand-held projector-based interface.

\begin{figure}[!h]
    \center
    \includegraphics[width=8cm]{pics/FittLaw.PNG}
    \caption{Crossing Fitt law: {\em variability is allowed in the direction orthogonal to movement} by Accot \cite{accot2002} }
    \label{FittLaw}
\end{figure}


This crossing principle is well described in the crossY study by Apitz and coll. \cite{apitz}. Figure \ref{crossY} compares the traditional and crossY way of selections. Apitz  wanted to compare the efficiency of crossing interaction with point-and-click by stylets. The idea was to avoid the alternation \textit{"between a very natural and fluid input mode for sketching or taking notes and a very rigid and segmented interaction while using the GUI elements"}. Crossing finally leads to a fluid composition of commands what is perfectly suitable for our eye interaction in which we want to use saccade more than fixation (used by dwell-time) because fixation is not something that human being is naturally doing.


The crossing interaction has already been used in some way for people with motor impairments and its efficiency have been tested on different modalities. Wobbrock \cite{wobbrock2007,wobbrock2008} shows in his papers that for disabled people interacting with the trackball, for example, it's easier and faster to handle a crossing interaction compared to a point-and-click interaction that needs more {\em sub-actions} and that needs the user to be really accurate. A smooth way of interacting, without needs of interrupting is hence really useful here. 
Crossing by eye tracker has also been tried, mainly for text-entry softwares, and have been considered as an interesting way to study in the Kurauchi text-entry system for example \cite{kurauchi2016,kurauchi2018}, because of its dwell-free property.
However, this last study can only be applied in a very restricted field (text-entry), compare to the design we want to create that would be something adapted to different situations (different selection menus for example) and, obviously, something that could be usable in an AAC system based on pictograms and images, instead of in a traditional "text" communication software what is something really specific.



\section{Communication with children with multiple disabilities}

In fact, the interaction we want to keep in mind would be, in the near future, improved and tested to interact with children with multiple disabilities. These children, as explained before, can have mental impairments that lead to almost impossible learning of basic text reading. The use of an AAC method is then a way to communicate efficiently with the children with intellectual and developmental disabilities as presented in the Chirvasiu \cite{chirvasiu_alternative_2018} or Sigafoos \cite{sigafoos_augmentative_2016} studies. The idea is to base the communication on several pictograms or images that have been taught to the child, and that is used by the parents, the doctors, and all the entourage of the children during the day, to represent objects, concepts or actions that they want to talk about. Several studies using these systems with the gaze have already been done and showed the power of AAC by gaze, we can count the Townend \cite{townend2016} study in a netherlander family with a daughter with a Rett Syndrome or the special case of M.B., a young girl also having a Rett Syndrome studied by Patachon \cite{patanchon2015} in 2015. Of course, the limitations here are the same as the ones quoted before, it's to say that the interaction remains really slow. 

The design we have to propose for this study hence have to be intuitive and easy to use, to be learned by the children who will need to use it daily, but also by their families and doctors to be "ecological" for next studies.  In order to be relevant in our current study the design of the interaction has to be easy and fast to handle for people with temporary invalidity due to an accident for example and it has to be really comfortable to use for the surgeon or any people who would need to use it on a long time period, as we first focus our research on people without disabilities. Later then, in another study, we will try to refine this interaction to make it more suitable for children with multiple disabilities especially.

For this study, the goal is therefore to design an interaction that is suitable for most of the people that have to use eye tracker technology daily, on short or longer period, by keeping in mind the fact that we will then try to extend it in particular case for people with strong disabilities, eventually by testing it through an AAC tool or by the creation of some games for children with multiple disabilities.




==> Master2Repport/chapters/3_Chapter3.tex <==
\chapter{Contributions}
\section{Implementation}
\subsection{Description of the design }

Our first idea, for the creation of this crossing menu, was to investigate the design of marking menus usable by eye-trackers. We quickly tested the drawing of a path with eye tracker and realized that a marking menu would be unusable with gaze: it’s not in the human eye nature to follow a homogeneous path with the eyes. 

We considered a circular pie menu which appeared to be a viable approach for an eyecrossing interaction. The circular shape of the menu was more suitable than the existing grid menu, mainly because a grid menu design would have led to triggering an action each time the user jumps from an element to another (crossing a line or a row of the menu). In other words, a grid menu would create another Midas Touch problem making the menu impossible to use. For the implementation of our interaction, we were inspired by the pEye menu design by Huckauf \cite{huckauf2007,huckauf20081} (cf fig \ref{pEyeA}). Our design had to be adapted to human gaze movement and suitable to our expectations of an explicit selection interaction. We believed in the fact that removing hierarchical constraint given by pEye and Quickwritting as much as possible was a good thing to have the fastest interaction possible. The concepts presented in these papers are really interesting because they stick to our initial idea of circular crossing menu, but they are unfortunately not giving a lot of valuable results due to some uncertainty in the pre-requisites of the designs and tests, like the optimal number of slices. 

The first thing we then have to do is to compute this maximal number of elements that can be placed on this menu. In the Urbina’s paper\cite{urbina2010} a 6 slices menu is considered as "optimal" without taking into account the width of the menu (and with only one specific eye-tracker), what seems to be however one of the most important variables to explore. Firstly then, we have to compute some more accurate values about the number of slices, depending on the menu dimension and on other important constraints like the eye-tracker. We then have to validate and improve the properties quoted by the initial paper (fast way of interaction, easy to understand, save time from the dwell, etc) and we have to test it on a bunch of people.

The final design used during user tests phase is hence a circular menu where each section contains an item. In order to select an item, the goal is to achieve a crossing interaction by moving our gaze from the section to the outside of the menu. The crossing event will be triggered somewhere between the boundaries of the menu item and a distance near to the menu.




\subsection{Assumptions }
\subsubsection{Allow easy exploration}

The crossing interaction in our menu will be triggered outside the menu. It means that inside the menu, the user should be able to freely explore the elements, without having some visual feedback pollution like with dwell-time, and without fearing an unwanted activation. We hope that this implementation could make the user feel less stressed by the use of the menu. In comparison with the dwell-time method, the crossing method creates a "break" {\em before} the selection, and not {\em during} the selection (while the user has to not move during the dwell-time). The user will first look for the element he/she wants to select, and then he/she will select it. These two actions can be done separately, or in one row, the user can choose, contrary to the dwell interaction that always has to be done in two steps. We also hope that the fact of letting the user select the object when he/she want will makes the selection more comfortable.

\subsubsection{Faster and less tiring than Dwell-Time}

The human eye is constantly moving a lot, doing saccades or micro-saccades. 
The use of dwell-time interaction can be hard to handle on small items because of that, eyes can, for example, move "unintentionally" due to the micro-saccades or it can be attracted by something in the peripherical view.

The fact of turning the action into a crossing interaction is more human-friendly because it will mainly use the saccade movement of the eye, what is one of the most natural movement it can achieve.
Eye saccade is accurate and not so tiring compared to focus. The action asked the user can become less stressful and less tiring because acquiring a target by crossing interaction doesn't necessarily ask the user to be as accurate as for "pointing" as Wobbrock showed with it's crossing/pointing comparison with mouse and trackball \cite{wobbrock2007}.
Also, when the crossing interaction is used in an expert mode, we think that a big part of the 500ms usually spent by the dwell-time can be saved during the activation leading to faster action.


\subsubsection{Size and number of sections in pie} \label{computation}

The eye-tracker used in this study, the {\em Tobii{\copyright}  4C} eye tracker, is considered as "well-calibrated" if, 93\% of the user test population results have a maximum offset of 0.8 degrees in accuracy and 0.5 degrees in precision\footnote{Tobii {\em Accuracy and precision test method for remote eye trackers}: https://www.tobiipro.com/learn-and-support/learn/eye-tracking-essentials/}, it's to say it has a total of 1.3 degrees of uncertainty when used at a distance from 50 to 95 cm to the user given by the {\em Tobii{\copyright}  4C } description \footnote{Tobii 4C description page: https://gaming.tobii.com/product/tobii-eye-tracker-4c/}. 
\newline

Let first consider a comfortable reading distance, usually settled between 38.1 to 63.5 cm, with a text written in a 12 pts size ($\approx$ 0.45 cm). 

We want to display a letter inside a circle or a square. To make it more readable we are adding a small margin between the letters and the border of its container, for a letter in size 12pts, the margin will also be equal to 12pts as shown on fig \ref{LetterSize}.

\begin{figure}[!h]
    \center
    \includegraphics[height=4.5cm]{pics/LetterSize.png}
    \caption{Position and size of the letter in the circular and rectangular box item.}
    \label{LetterSize}
\end{figure}


By considering the mean comfortable distance between 38.1 and 63.5 cm and knowing the working distance of the eye tracker, we consider a comfortable distance between 50 to 63.5 cm. Using the fig \ref{angle} we can see that the angle is about:


\[ angle = 2 \times \frac{angle}{2} = 2 \times atan(\frac{\frac{3 \times CharacterSize}{2}}{ComfortableReadingDistance}) = 2 \times atan(\frac{\frac{3 \times 0.45}{2}}{\frac{50+63.5}{2}}) \approx 1.36\textrm{ degrees} \]

\begin{figure}[!h]  
    \center 
    \includegraphics[height=4.5cm]{pics/angle.png}
    \caption{Computation of the vision angle using comfortable reading distance and size}
    \label{angle}
\end{figure}


Obviously, comfortable vision angle is greater than the Tobii{\copyright}  uncertainty angle (1.36 degrees > 1.3 degrees). Therefore we can see that the limitation of our design in term of element size should be given by the human eye comfort itself.
\newline

Now that we have the distance angle for one object, let's take a user with 10/10 corrected on each eye at a distance from 50 to 60 cm from the eye tracker. We can compute the maximal number of item composing a menu giving the dimensions of this menu.By taking the maximal degree of uncertainty given by the eye comfort limitation we can deduce the minimal size of a selectable object on the screen.

Let's consider first a circular menu with a radius R, the perimeter of the radius is

\[perim = 2 \times \pi \times R\]

The minimum object size at a distance D to the user can be computed geometricaly as shown in the fig \ref{objSize} :

\[objSize = 2\times D\times tan(\frac{angle}{2}) \]

\begin{figure}[!h]  
    \center 
    \includegraphics[height=4.5cm]{pics/objSize.png}
    \caption{Computation of the minimum object size at a distance D using a given vision angle }
    \label{objSize}
\end{figure}

For a user at a D distance from a circular menu of radius R, we obtain a maximal number of slices, as explained with the fig \ref{sectionNumberC}, equal to: 

\[ \theta = 2 \times asin(\frac{\frac{objSize}{2}}{R\times2})\]

\[ arcLength = \frac{perim}{360} \times 2 \times \theta \]

\[ numberOfSlices = \left \lfloor \frac {perim}{arcLength} \right \rfloor \]

\begin{figure}[!h]  
    \center 
    \includegraphics[height=4.5cm]{pics/slicesNumber.png}
    \caption{ Computation of the maximum number of slices for objects with a givein size in a circular menu }
    \label{sectionNumberC}
\end{figure}


This computation can complete the Huckauf and Urbina's study\cite{urbina2010} about the limits of the number of slices in pEYEs menus by proposing a formula taking in account the radius of the menu, the distance to the user and the angle used as spacial accuracy, and giving the maximal number of slices that can be represented in a menu.
\newline\newline

Now, in order to design a comparative study with the STATUS QUO dwell-time based menus, we also need to compute the size of a grid menu for a given number of elements, to be able to implement it. We decided to use square elements and to take a design where the number of rows equals to one-third of the number of columns what leads to the fact that width of the grid equals 3 times the height (cf fig \ref{sectionNumberL}). The object dimensions for a square object is then equal to $objSize \times objSize$. It means that for a menu of Width $W$ we have a maximum number of objects equal to :

\[ numberOfElements = \left \lfloor\frac{W}{objSize}\right \rfloor \times  \left \lfloor\frac{\left \lfloor\frac{W}{objSize}\right \rfloor}{3}\right \rfloor \]

\begin{figure}[!h]  
    \center 
    \includegraphics[height=4.5cm]{pics/sectionInGrid.png}
    \caption{Computation of maximum number of element in grid menu with a given width}
    \label{sectionNumberL}
\end{figure}

We are also assuming that the main area taken by the circle crossing menu compared to the grid dwell menu is bigger for the same number of objects could become a problem if we need to represent too many elements in the menu.
   

==> Master2Repport/chapters/4_Chapter4.tex <==
\section{Design of the User experiments}

We conducted a user experiment to observe and measure the benefitts and drawbacks of crossing-based gaze activation.

\subsection{Experiment design}
\subsubsection{Participants}

As motivated in the introduction, we conducted an initial study with participants having no disabilities.

We invited 19 volunteer students to participate in the study. They are aged from 21 to 33 years old and come from 7 different nationalities. 15 of them are Master students in computer sciences, 2 of them are Master students in history, and 2 others are Ph.D. students in computer sciences. Among all the participants, 4 of them had already used an eye-tracker before. The data from one participant was dropped because he/she was colorblind and thus unable to distinguish the colors for ``correct'' and ``incorrect'' validations. This raised our attention to work on a better use of colors in our system.

\subsubsection{Apparatus and Environment}

Experiment are performed in a bright room with no artificial light. Participants are sitted between 50 and 60 cm from the {\em Tobii 4c } eye tracker placed at 75 cm height from the floor. The tracker is connected to a {\em MacBookPro{\copyright}  11.3 Intel Core{\copyright}  i7-4980 HQ} running under the {\em Windows{\copyright} 7 pro 64 bits } OS with 16 Go of RAM. Testers are asked to sit comfortably and to try not to move during the test phase. For each participant, an initial gaze tracking calibration is done at the beginning of the test session. This calibration starts with the {\em Tobii{\copyright} eye tracking software} of {\em the Tobii{\copyright} 4C eye tracker}, followed by another calibration that we developped. This second calibration reduces the eye tracker accuracy offset before each of the different tests. It works by compensating the average offset of 5 different points on the screen (top-right, top-left, bottom-right, bottom-left and center).

\subsection{Design of the experiment's menu}

\subsubsection{Global appearence} 

Giving the distance between the user and eye tracker and giving the pre-computed object size, we want to create two kinds of menu representing the two {\em experimental conditions} in our studies. The first menu in the STATUS QUO condition is similar to the ones used in various existing aided AAC grid selection systems using dwell-time (e.g. fig. \ref{snapCore} by Tobii Dynavox\footnote{Tobii Dynavox Snap+Core description page: https://www.tobiidynavox.com/en-US/software/windows-software/snap/}).
For {\em ecological} concerns, we created a 27 elements grid representing the 26 letters of the Latin alphabet and an empty slot used as a text field to display information during the tests. \sr{expliquer que nous avons préféré ça à <détailler> qui aurait été davantage contrôllé mais moins écologique. Ça montre que nous avons pensé à la solution plus contôllée, que ce n’est pas un oublié, mais bien un choix délibéré.} We choose to use the Latin letters as elements of the menu because they are symbols that are known by all of the testers. In normal use, the user would have an idea in mind and would have to search for the corresponding element in the menu. If he/she is not a novice user, she would be able to approximately or exactly determine the position of the element needed. The fact of using letters is useful here because they can be sorted easily (by using the alphabetical order) in order to simulate this expert (or at least not novice) knowledge of the item position on the design. The use of other elements like images would have lead to find a way to help the user to find the elements, or otherwise we would have faced a long search time distorting the main result, in both cases, these implementations would have lead to a more controlled solution, what was not the the goal of this paper.  The final design of the grid menu is represented in figure \ref{dwellMenu}. We added some feedbacks to the menu when an object is being looked by the user, the cell containing the object turns to yellow and a progress circle is displayed to give the dwell-time feedback.
\newline\newline

\begin{figure}[!h]  
    \center 
    \includegraphics[height=4.5cm]{pics/DwellMenu.PNG}
    \caption{Dwell grid menu with the 26 letters of the latin alphabet in alphabetical order.
    The central slot will be used as text field during tests.}
    \label{dwellMenu}
\end{figure}

 

The second menu in the CROSSING condition is the circular menu with crossing interaction that we created.
We noticed during the pre-test sessions that the pEye interaction was a bit hard to use for some people. It was hard for them to go beyond the boundaries of the menu intentionally to activate the outside crossing area (they were "blocked" inside the menu). To solve this problem and to ease the action we added circle targets outside of the menu, one for each section, in order to create a visible target for the user to help him/her to go outside of the menu and so to cross the crossing area more easily. The main design of our circular menu and the target circle can be seen below on figure \ref{crossingMenu} such as the circles used as target. As we can see the addition of these new targets is also taking some space on the screen so it will have to be taken into account for future implementations.

\begin{figure}[h!]
\centering
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=6cm]{pics/CrossingMenu.PNG}
  \caption{}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=6cm]{pics/CrossingTarget.PNG}
  \caption{(i) disk target. (ii) invisible crossing area}
\end{subfigure}
\caption{(a) Main design of the circular crossing menu. (b) Close-up on the disc targets displayed to ease the crossing interaction.}
\label{crossingMenu}
\end{figure}


\subsubsection{Menu sizes} 

By using the object size computed in the part \ref{computation} for a user sitting at a distance from 50 to 63.1 cm from the eye-tracker, we compute the size of the two different menus with 26 elements. 


\begin{itemize}

\item for circular crossing menu the radius of the menu is 
\[ CrossingMenuRadius = \frac {objSize}{4 \times tan(\frac{360}{4 \times 26}) } \approx \frac {1.31}{4 \times tan(\frac{360}{4 \times 26}) } \approx 5.37 \textrm{cm}\]

\item for grid dwell menu the dimension of the menu are
\[ DwellMenuWidth = 9 \times objSize \approx 9 \times 1.30 \approx 11.7cm\]
\[ DwellMenuHeight = 3 \times objSize \approx 3 \times 1.30 \approx 3.9cm \]
\[\textrm{(because} \quad 26 = 9 \times 3 -1 = (3\times 3) \times 3 - 1 \textrm{)}\]

\end{itemize}


\begin{figure}[!h]
    \center
    \includegraphics[width = 10cm]{pics/snapCore.jpg}
    \caption{{\em Snap+Core by Tobii Dynavox}, an example of AAC grid system. }
    \label{snapCore}
\end{figure}


\subsection{Task}

\subsubsection{{\em Search and Select} Task}

For the first task, we want to observe the mean time spent by the user to search for, consider, and select a given item. In both the STATUS QUO and CROSSING conditions, we display the prescribed item in the middle of the menu (cf fig \ref{menuSearch}). The participant has to search for it in the grid or in the circle and to activate it. We asked participants to perform the task as fast as possible while avoiding errors (i.e. selecting a letter different from the prescribed letter). As the dependent variable, we recorded \verb+activation time+: the time between the apparition of the prescription and the activation of the letter by the participant. For further analysis, we also recorded the time spent by the user to go back to the center of the menu after activation to prepare for the next trial.

\begin{figure}[h!]
\centering
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[height=3 cm]{pics/DwellMenuSearch.PNG}
  \caption{Dwell menu {\em Search and Select} test design.}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[height=4.5cm]{pics/CrossingMenuSearch.PNG}
  \caption{Crossing menu {\em Search and Select} test design.}
\end{subfigure}
\caption{The center area is used to display the next letter the user have to search.}
\label{menuSearch}
\end{figure}

Participants perform 3 blocks of search and select trials. Blocks are used to offer relaxation time for the eyes (between blocks) and to observe a possible learning effect during the experimental session. In each block, participants have to look at 55 letters in a pseudo random order. Each of the 26 letters appears exactly twice except for the 3 first letters that appear 3 times. These first 3 letters are used as a warm-up and are not counted in the final results.



\subsubsection{{\em Selection} Task}

\begin{figure}[h!]
\centering
\begin{subfigure}{\textwidth}
  \centering
  \includegraphics[width=14 cm]{pics/consignes.PNG}
  \caption{Exemple of text asking the user to alternately select two letters.}
\end{subfigure}
\centering
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[height=3 cm]{pics/DwellMenuSelect.PNG}
  \caption{Dwell menu {\em Selection} Test design}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[height=4.5cm]{pics/CrossingMenuSelect.PNG}
  \caption{Crossing menu {\em Selection} Test design}
\end{subfigure}
\caption{The user need to alternately select ten times several each of the  couples of letters previously given by the program.}
\label{menuSelect}
\end{figure}

The previously described ``search and selection task'' requires participants to search for a letter, which can lead to high variability in the final \verb+activation time+. We were also interested in the {\em raw} efficiency of the crossing selection for target activation, i.e. activations that do not require an initial search. Activation without search also has strong ecological validity: when becoming expert of a system, we often need to activate targets for which we know the precise location.

We designed a reciprocal {\em Selection} Test (fig \ref{menuSelect}) to remove most of the {\em observation} and {\em search} time required for the target activation. Participant have to activate two letters alternately with 10 repetitions (i.e. 20 activations). Before starting a trial, we ask participant to locate the two letters that they will have to activate.
We vary the two letters in each trial in order to control their relative distance; which has an impact of activation time. As in the previous task, we use the two first activations of a trial as a warm-up and we don't count it in the final result.
\newline 


==> Master2Repport/chapters/5_Chapter5.tex <==
\section{Results}
\subsection{Data pretreatment}
Due to a bad implementation of blinking detection on Tobii eye-trackers, it was hard to remove blink unexpected movements from the final dataset. We hence decided to remove all the data receiving an error from the user to delete most of the unexpected actions. We hence use only the good attempts to mainly focus on the interraction itself an not on the general designs. Usually, a blinking is leading to a big move to the bottom following by a movement going back to the initial position, for items being around the bottom part of the menu it can fastly lead to an unexpected activation.
Of course, due to this blinking problem, the error rate of each participant can be really high (more than 10 \%) but could be obviously reduced significantly by having a good implementation of the blink detection.

\subsection{{\em Search and Select} Test results} 
\subsubsection{Comparison between methods}

\begin{figure}[h!]
\centering
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=8cm]{stats/User_Dwell1_VS_Crossing1_QS.png}
  \caption{Time to select an element when user know it.}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=8cm]{stats/User_Dwell1_VS_Crossing1_SQ.png}
  \caption{Time to go back to the center of the menu.}
\end{subfigure}
\caption{Time results by user for session 1: Dwell-time VS Crossing}
\label{cvl1}
\end{figure}

On the first session (cf fig \ref{cvl1}), we compare, for the two menus, the time taken by the user to activate an element after he/she saw it in the middle of the menu, and the time taken to go back to the middle of the menu after he/she activated it. We can clearly see at first that the time spent to search for an object and to activate it is way longer than the time spent to go back to the middle of the menu after having activated this object (about 1 second more). The path needed to go from the middle to an element or from an element to the middle being approximately the same, the search and activation time is hence obviously the most important part of the time spent by the user during the selection phase. 

Then we see that the time spent to go back to the center of the menu on the crossing menu is longer than the one on dwell-time menu in 10/12 cases. This difference of time could be due to the distance to the center that is different but also to the direction of the eye movement (we know that a top-down movement is faster than a bottom-up movement), also the users are maybe more used to linear menus. 

For the Search and Select part, the crossing interaction is faster in half of the cases, even if we can see that for candidates 1 and 12 the times are really close. We can already notice that for people having already use an eye tracker before (candidate 1,2 and 6 ), the time for crossing is either better, either really similar to the time for dwell. In both cass they seems to be faster than other testers. 

In both graphs we can notice that there seems to have some unexpected values, they could be due to some problem of eye-tracker calibration or some eye tiredness during the exercise. What we can also notice is that people who started with dwell time (1,2,3,5,6 and 10) tend to have better results with crossing whereas people who started with crossing (4,7,8,9,11 and 12) tend to be faster with dwell. It can significate that they probably can both learn from one or the other method, and so they become faster on the second test.

\begin{figure}[h!]
\centering
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=8cm]{stats/User_Dwell2_VS_Crossing2_QS.png}
  \caption{Time to select an element when user know it.}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=8cm]{stats/User_Dwell2_VS_Crossing2_SQ.png}
  \caption{Time to go back to the center of the menu.}
\end{subfigure}
\caption{Time results by user for session 2: Dwell-time VS Crossing}
\label{cvl2}
\end{figure}

For the second session (cf fig \ref{cvl2}), 5/12 people only are faster with crossing for the  Search and Select time, still including people having used eye-trackers before. We can also notice that they are still mostly faster than other testers with both techniques.

For the fact of going back to the center after activation, we can see that 11 of the 12 people are faster with the dwell menu. Except for case 10, they also tend to be a bit more regular on crossing menu than on dwell menu. It's an interesting property probably showing that the users have good learning of the menu center, it could be useful to use this information in another design.


\subsubsection{Improvement between sessions}

\begin{figure}[h!]
\centering
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=8cm]{stats/User_Dwell1_VS_Dwell2_QS.png}
  \caption{Time to select an element when user know it.}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=8cm]{stats/User_Dwell1_VS_Dwell2_SQ.png}
  \caption{Time to go back to the center of the menu.}
\end{subfigure}
\caption{Time results by user for both sessions: Dwell-time }
\label{c}
\end{figure}

By comparing the sessions 1 and 2 for the dwell menu (cf fig \ref{c}), we can see important learning of the interaction: on the  Searching and Selection, most of the people (11/12) are faster on the second session and more regular (8/12). They are also all faster on the 2nd session for the action of going back to the center of the menu meaning that they are also learning the design of the menu.

\begin{figure}[h!]
\centering
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=8cm]{stats/User_Crossing1_VS_Crossing2_QS.png}
  \caption{Time to select an element when user know it.}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=8cm]{stats/User_Crossing1_VS_Crossing2_SQ.png}
  \caption{Time to go back to the center of the menu.}
\end{subfigure}
\caption{Time results by user for both sessions: Crossing }
\label{l}
\end{figure}

In the same way, for the second crossing session (cf fig \ref{l}), people are all faster and regular (except for the unexpected value of tester 10) for going back to the center of the menu so we can assume that their is a real learning of the design of our menu. On the other hand, the learning rate of the {\em Search and Select} actions seems to be a bit lower because only 8/12 people are faster on the second session and around half of them are more regular. It can significate that to become faster on this kind of menu a longer training period could be needed. We can notice the fact that expert testers (i.e. people having use an eye tracker before the test sessions) are still improving there times on the second session so they could potentialy become even faster with more training.

\begin{figure}[h!]
\centering
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=8cm]{stats/User_Mean_QS.png}
  \caption{Time to select an element when user know it.}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=8cm]{stats/User_Mean_SQ.png}
  \caption{Time to go back to the center of the menu.}
\end{subfigure}
\caption{Mean time for both session with Dwell-time and Crossing methods}
\label{mean}
\end{figure}

When focusing on the mean values of the candidates for the two sessions of the two menus (cf fig \ref{mean}), we clearly see that even if the time spent to go back to the middle of the menu is lower on the second session for both menus, it is always longer on the circular menu. Anyway, crossing also seems to have a bigger learning rate so maybe a few more training would leadd to a better result by using the crossing menu than by using dwell-time. For the  Search and Select time, on the first session the crossing interaction seemed to be slightly faster (with a bigger irregularity) but it unexpectedly slows down on the second session contrary to dwell that speeds up and so become faster. 

Regarding the previous graphs, an explanation for these results could be the fact that people who were not used to eye tracker can become tired with thess methods. In fact, people having a slower time on session 2 for crossing are either people who started with dwell-time menu and who said that it was still hard for them to use fastly the crossing menu at the end of the tests (candidate 3 and 10) or people starting with crossing who were not used to eye tracker and who may have needed more time to learn how to use it efficiently (candidate 9, 12).

\subsection{{\em Selection} Test results}

\subsubsection{Comparison between methods}

In the real conditions of use, the user will not have to look at the center of the menu before selecting an item. We believe that removing this useless action would lead to a faster activation of elements on crossing menu that's why we designed the following tests. For this new series of tests based only on the selection, we computed the mean time of selection by the user depending on the selection method by alternating the selection of several couples of letters.

\begin{figure}[h!]
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[height=5.5cm]{stats/User_Alternate_Global2.png}
  \caption{Time by user to select one letter.}
\end{subfigure}%
\begin{subfigure}{.6\textwidth}
\hspace{.35\textwidth}
  \includegraphics[height=5.5cm]{stats/ratioa.png}
  \caption{Ratio between Crossing and Dwell selection time.}
\end{subfigure}
\caption{Time comparison between Dwell-Time and Crossing methods for the {\em Selection} Test.}
\label{s}
\end{figure}


What we can observe with the results of fig \ref{s} is the fact that among the 6/11 people faster with the crossing, 4 of them are the people who had already used an eye tracker before (2,4,8,9), and they are faster than all the others (about 100 ms faster on dwell and usually more than 200 to 300 ms on the crossing). We can also notice that they are faster with crossing than with dwell-time.

Actually, more generally we can see that a person fast and regular with the two methods (meaning that he/she learned how to use the eye tracker) tends to be faster with the crossing method. We actually have an exception with candidate 3 who clearly said that it was "particularly boring" to alternate the selection for two elements near to the other on the circular menu. What the ratio between crossing and dwell says is that for a "random" set of user we have approximately the same speed using one or the other menu. But actually, when looking at the special case we see that it really depend on the user's profile.

\begin{figure}[h!]
\centering
\begin{subfigure}{.4\textwidth}
  \centering
  \includegraphics[width=5.5cm]{stats/dwellletters.png}
  \caption{Mean time for the couples of letters of the Dwell-time menu }
\end{subfigure}\hspace{.1\textwidth}%
\begin{subfigure}{.4\textwidth}
  \centering
  \includegraphics[width=5.5cm]{stats/crossingletter.png}
  \caption{Mean time for the couples of letters of the Crossing menu}
\end{subfigure}
\caption{Mean time of selection for one letter of the different couples of letters during the {\em Selection} Test for both Dwell-time and Crossing methods.}
\label{letterstime}
\end{figure}

By looking at the data in details we noticed that the disposition of a couple of letters (cf fig \ref{letterstime}) can have an impact on the selection time for the crossing menu. For example, a couple of letters on the diagonal of the crossing menu, A-N and G-T, will be selected faster than other couples for example. In the other side for dwell time, H-I and J-R, the couple having letters near the one to the other, will result in a faster selection. This information can be really useful in order to sort the items of each of the menu. For example, we can decide to put two items that are usually activated the one after the other the farthest possible in the circle of the crossing menu in order to have a faster interaction.

\begin{center}
   \begin{tabular}{ | c | c | >{\centering\let\newline\\\arraybackslash\hspace{0pt}}m{3cm} | >{\centering\let\newline\\\arraybackslash\hspace{0pt}}m{3.5cm} |}
     \hline
     \multicolumn{4}{|c|}{Recapitulative Table} \\ \hline
    \multicolumn{4}{|c|}{{\em Search and Select} Tests} \\ \hline             	
    \multicolumn{2}{|c|}{Test Comparison} & Users faster with (b) method &Expert users faster with (b) method \\ \hline
     \multirow{2}{*}{\shortstack{Session 1: (a) Dwell \\ VS (b) Crossing}} & object selection & 50\% (6/12) & 66.67\% (2/3) \\ \cline{2-4}
     & back to center & 16.67\% (2/12) & 66.67\% (1/3)\\ \hline
     \multirow{2}{*}{\shortstack{Session 2: (a) Dwell \\ VS (b) Crossing}} & object selection & 41.67\% (5/12)& 100\% (3/3) \\ \cline{2-4}
     & back to center & 8.33\% (1/12) & 33.33\% (1/3)\\ \hline
     \multirow{2}{*}{\shortstack{(a) Dwell session 1 \\ VS (b) Dwell session 2}} & object selection & 91.67\% (11/12) & 100\% (3/3) \\ \cline{2-4}
     & back to center & 100\% (12/12) & 100\% (3/3)\\ \hline
     \multirow{2}{*}{\shortstack{(a) Crossing session 1 \\VS (b) Crossing session 2}} & object selection & 66.67\% (8/12) & 100\% (3/3)\\ \cline{2-4}
     & back to center & 100\% (12/12) & 100\% (3/3)\\ \hline
     \multicolumn{4}{|c|}{{\em Selection} test} \\ \hline
     \multicolumn{2}{|c|}{Test Comparison} & Users faster with (b) method & Expert users faster with (b) method \\ \hline
     \multicolumn{2}{|c|}{(a) Dwell VS (b) Crossing} & 55.54\% (6/11) & 100\% (4/4)\\ \hline
   \end{tabular}
 \end{center}

\subsection{Users feedbacks}

After the tests sessions, users were asked to freely express their feelings about the different techniques and to say why they preferred to use one or the other.

Among the 16 users, 8 of them had a preference for the crossing menu, 5 others prefer the dwell-time menu and the 3 last ones didn't have a real preference.
\newline\newline
People preferring crossing interaction said that dwell-Menu can be "frustrating" and "stressful". During the search/observation phase "the display of the dwell feedback is disturbing", "it catches the attention" and the dwell time is generally considered as "too short", leading to some selection errors. User needs to "keep the eyes moving" what is stressful and tiring. In another side, during the selection phase, the dwell-time is considered as "too long", leading to an impression of a waste of time and making the user "unable to think to his/her next action". The crossing menu creates the feeling of a faster interaction it is less frustrating because the user "don't have to rush", he/she "can relax his gaze without activating any element". The menu is bigger for crossing so it needs bigger movement but it seems to be useful to do fewer errors and it can become a problem if we want to add more elements.
\newline\newline
For the people who preferred the dwell interaction, they explained that "even if dwell-time can lead to more error" it generally seems to be "more explicit" than the crossing interaction and can be understood more easily. Because of that, one of the users said that "by training more on the crossing he really believes that he could become faster", the interaction was just "not enough explicit" for him and he feels like he needs more time "to deal with it". Testers also said that it seems to be faster and a bit "more comfortable" because fewer eyes movements are needed, "especially when two letters are near the one to the other". 


==> Master2Repport/chapters/6_Chapter6.tex <==
\chapter{Conclusion}
The current eye-tracking interaction methods are still not explicit enough and so they still face the Midas Touch Problem. Event if the Dwell-Time interaction is considered as quite efficient and tend to reduce this problem with the use of various techniques, like automatically adjustable dwell-time, the problem never completely disappear. Moreover, the use of dwell-time can become a big waste of time for people having a lot of eye-tracking interactions, because each selection leads to a small waiting time during the dwell. The goal of this study was to create a new interaction method by eye trackers that suits people having to daily use it on a short or long period.  
In order to find a way to reduce the drawbacks of eye-tracking interactions, we inspired from several studies, like the pEye design of Huckauf \cite{huckauf2007,huckauf20082},  to create a circular crossing menu usable by eye-tracking methods. We tried to keep in mind the possibility of a future adaptation of our design for children with some multiple disabilities who have to daily use these kinds of devices and interaction methods, especially to communicate with others. It is hard for people having to use an eye-tracking system as a mean of communication to express themselves, the action is slow and can then become frustrating.
\newline\newline

The use of crossing is useful to give a neutral area to the user in order to relax his/her gaze, what should tend to avoid the tiredness and the stress due to the actual interaction. The main idea was actually to use the crossing method in order to have a “direct” interaction making us able to completely remove the time wasted by the Dwell-time during the selection and feeling more natural to the user. We also thought about the use of a circular menu instead of a linear one in order to avoid the Midas touch problem with crossing (the elements are selected when crossing the boundaries of the menu, not when going from an element to another).
\newline\newline

As explained in the paper, our design still has some limitations. A blink-proof algorithm should be added to our technique in order to lower the error rate which is too high for our crossing interaction. It could lead to better use of the system and would permit to exploit more data. For now, the non-implementation of this algorithm can disturb the user and is potentially a cause of the slower interaction for the « novice » users, i.e. for users who never use eye-trackers. 
We may also need to rearrange the shape of our menu. The fact that the time taken to come back to the center of the menu in the {\em Search and Select} Test was longer for our crossing menu showed that the shape and the size of the design were probably influencing the general time of activation of the elements. A study on different kinds of shape for crossing menu could be interesting to work on, comparing the activation time between the different designs of the menus (Circular, Elliptique, Square, etc).
Some more specific modifications could also improve the performance of some users. Effectively, we noticed that people who were generally slower on the {\em Selection} Test tend to be really faster on the dwell-time interaction compare to the crossing. It seems that the dwell is easier to learn for some “novice” testers and can be handled more easily. Our interaction was considered as not explicit enough for some people. Moreover, we realized that our model was not colorblind-proof. Work on the colors of the different elements of the menu and on feedbacks is then needed to avoid these kinds of problems. 
However, the general results of this study are really promising. The crossing interaction seems to effectively be as efficient as dwell time for most of the people who never used an eye tracker before. As we explained for some of them it was a bit harder to handle the crossing interaction, because of this “un-explicitness”, but some of them explicitly said that with few more training they thought that they could become faster on crossing and probably faster than dwell-time, because of the “direct” interaction, as we were expecting. 

About the testers who were the most interesting for future studies, i.e. people having already use an eye tracker and knowing how to deal with it, it seems that our proposed method is well-adapted. These people have the best time results on each of the different tests and our interaction induce a faster way of selection compared to the dwell-time {\em statu quo}. As novice users thought, we believe that longer use of eye trackers could increase the speed of all the users. Another study on a longer test period would then be useful in order to test this hypothesis. It's already a big improvement to see that an alternative to the dwell-time seems to be possible for people using an eye tracking system and to see that this alternative look more efficient for expert users of eye-trackers.
\newline\newline

This study can be seen as the complementary step of the {\em Gazeplay} project\footnote{Gazeplay website and git: http://www.gazeplay.net/ ; https://github.com/schwabdidier/GazePlay} \cite{schwab}, created in 2016 by Didier Schwab. The main idea of {\em Gazeplay} was to propose a low-cost software and game platform for children with multiple disabilities usable by eye-tracker. The cost of current technologies being expensive, this project was compatible with cheaper devices like the {\em Tobii 4C} and was giving a free open source software platform for the family and medical centers. In addition to be useful to make the children with multiple disabilities able to play "freely", the creation of this platform was aiming to teach and improve slowly eye-tracking interaction skills of these children. Our idea would be to integrate the interaction created in this study in some {\em Gazeplay}  games in order to test it with the children with multiple disabilities who are some of the people having the most interest in this new interaction technique. 
\newline\newline

The next important project related to our work is the AugCom project, under the direction of Didier Schwab, in partnership with Amélie Rochet-Capellan and Marion Dohen that should start in 2019. 
Communication through pictograms is required for lots of people who are unable to express themselves by word or gesture for short and long periods of time. There are currently various commercial software packages integrating eye-tracking but they don't really take into account the research results and objective evaluation of their system is usually missing.  The {\em AugCom} project aims to first do the state of the art of these software and its use, then it will more especially study the use of one of this software by adapting it to 3 children with multiple disabilities. Finally, the project will specify a software that will allow testing new hypotheses of interaction and composition of communicative messages. In the long term, this software will be available for the scientific community but also for the people concerned to help them in their daily communication. If the previous tests on Gazeplay were successful we could think about using our crossing method as the main interaction for this kind of projects.
\newline\newline

Moreover, the VR and AR devices being more and more present on the market, eye tracking technology seems to be the next step to add new features to these head mounted devices. After its integration in the well-known {\em HTC VIVE} Headset \footnote{Tobii Pro VR HTC Integration page: https://www.tobiipro.com/fr/domaine-dapplication/virtual-reality/}, the {\em Tobii} and {\em HTC} company, respectively leader in the eye-tracking and virtual reality fields announced their collaboration\footnote{{\em Tobii and HTC Bring Eye Tracking to Next Generation VR Headset}: https://www.tobii.com/group/news-media/press-releases/2019/1/tobii-and-htc-bring-eye-tracking-to-next-generation-vr-headset/} in the beginning of this year 2019 for the all-new {\em Vivre Pro Eye} \footnote{Vive Pro Eye website: https://enterprise.vive.com/us/product/vive-pro-eye/}, a new VR Headset integrating the eye-tracking technology. We can imagine that the AR could follow the same idea, regarding the {\em Tobii Glass pro 2} \footnote{Tobii Pro Glass 2 website: https://www.tobiipro.com/fr/produits/tobii-pro-glasses-2/} and {\em Tobii AR} \footnote{Tobii AR website: https://ar.tobii.com/} technologies proposed by the company. It could be really interesting to integrate our selection method in such devices in order to create a real fast portable hand free interaction system. We could think about all the different applications that could result in this integration: telecommunications, neuroscience, video games, augmentative and alternative communication, etc... 

Our study is opening lots of new opportunities to test on different devices and in different fields, each of them could lead to a significant improvement in the use of eye-tracking technology.

==> Master2Repport/chapters/7_Chapter7.tex <==
\chapter{Future work}

\section{Other implementations}

\subsection{Explore the design modification}

\subsubsection{A blink-proof implementation}

As explained in the paper, a blind-proof algorithm should be added to our technique in order to lower the error rate in our crossing interaction. It could lead to a better use of the system and would permit to exploit more datas.

\subsubsection{Colors and feebacks tests}

As we have seen during the tests sessions, our model is not colorblind-proof and some feedbacks doesn't seem to be explicit enougth for some users. Some more work on the color of the different elements of the menu and feebacks is then needed to avoid this kind of problems. We could think about an "exctension" feedback in wich the section gazed by the user could become bigger, it could be also usefull in our idea of AAC system in order to allocate more space to the pictures that the user is looking at.

\subsubsection{Shape arrangement}

The fact that the time taken to come back to the center of the menu in the {\em Search and Select} Test was longer for our crossing menu showed that the shape and the size of the design were probably influencing the general time of activation of the elements. A study on different kinds of shape for crossing menu could be interresting to work on, comparing the activation time between the different designs of the menus (Circular, Elliptique, Square, etc).

\subsection{Adaptation to other devices and integration in applications}

\subsubsection{Head Mounted Softwares}

The VR and AR devices being more and more present on the market, eye tracking technology seems to be the next step to add new features to these head mounted devices. After its integration in the well-known {\em HTC VIVE} Headset \cite{tobiivrdevice}, the {\em Tobii} and {\em HTC} company, respectively leader in the eye-tracking and virtual reality fields announced their colaboration in the begining of this year 2019 for the all-new {\em Vivre Pro Eye} \footnote{https://enterprise.vive.com/us/product/vive-pro-eye/}, a new VR Headset integrating the eye-tracking technology. We can imagine that the AR could follow the same idea, regarding the {\em Tobii Glass pro 2} \cite{tobiiardevice} and {\em Tobii AR} \cite{tobiiarsite} technologies proposed by the compagny.

It could be really interesting to integrate our selection method in such devices in order to create a real portable hand free interaction system. We could think about all the different applications that could result on this integration, telecomunication, neuroscience, video games, augmentive and alternative communication etc... 

 
 
 
\section{{\em AugCom}, an AAC project }
 
\subsection{Previous Step: {\em Gazeplay}}

The {\em Gazeplay} project \cite{schwab, gazeplay}, created in 2017 by Didier Schwab, can be seen as the prologue of this study. The main idea of {\em Gazeplay} was to propose a low-cost software and game platform for children with multiple disabilities. The cost of current technologies beeing expensive, this project tend to use cheaper eye tracker with the {\em Tobii 4C} and is giving a free open source software platform for the familly and medical centers. 
In addition to be something important to make the children having multiple disabilities able to play "freely", creating games for these children was a choice taken in order to teach and improve slowly eye tracking interaction to create in a near futur a fast alternative and augmentative eye tracker based communication software for people with multiple disabilities.

The idea for now, would be to use the interaction created in this study on the {\em Gazeplay} platform, by creating games using our new technique, in order to test it with the people that have the most interest in this new interction technique. The main goal by testing different kind of interaction with the children would be to find the most valuable one, (fast and confortable).

\subsection{Next Step: {\em AugCom} implementation}

Communication through pictograms is required for lots of people who are unable to express themselves by word or gesture for short and long periods of time. There are currently various commercial software packages integrating oculometry but they don't really take into account the research results and an objective evaluation of their system is usually missing. 

The {\em AugCom} project aims to first do the state of the art of these softwares and its use, then it will more espcially study the use of one of these softwares by adapting it to 3 children with a multiple disability. Finally the project will specify a software that will allow to test new hypotheses of interaction and composition of communicative messages. In the long term, this software will be available for the scientific community but also for the people concerned to help them in their daily commuication.
